The Elliptic Drinfeld Center of a Premodular Category

Given a tensor category C, one constructs its Drinfeld center Z(C) which is a braided tensor category, having as objects pairs (X, lambda), where X in Obj(C) and lambda is a half-braiding. For a premodular category C, we construct a new category Zel(C) which we call the Elliptic Drinfeld Center, which has objects (X, lambda1, lambda2), where the lambda i's are half-braidings that satisfy some compatibility conditions. We discuss an SL2(Z)-action on Zel(C) that is related to the anomaly appearing in Reshetikhin-Turaev theory. This construction is motivated from the study of the extended Crane-Yetter TQFT, in particular the category associated to the once punctured torus.

==> mytikz_macros.tex <==

\def\avgtwo#1#2{\fpeval{(#1+#2)/2}}

% I can't seem to get this to work to style nodes
% \DeclareRobustCommand{\mynodestyle}{circle}
% this is how to do it
%  (see answer in https://tex.stackexchange.com/questions/42800/global-variables-for-all-tikz-drawings-in-a-document)
\tikzset{
  mynodestyle/.style={
    circle, fill=white, draw, inner sep=1pt
  }
}


% defining local variables...
% this is too painful a way to define variables...
% note: it seems you can't have numbers in the var name...
%   \pgfmathsetmacro{\x}{0};

% braiding two strands
% input: x1,x2,y1,y2
\def\Braid(#1,#2,#3,#4){
  \draw (#2,#3) to [out=90,in=270] (#1,#4);
  \draw [white, line width=2mm] (#1,#3) to [out=90,in=270] (#2,#4);
  \draw (#1,#3) to [out=90,in=270] (#2,#4);
}

\def\BraidRev(#1,#2,#3,#4){
  \draw (#1,#3) to [out=90,in=270] (#2,#4);
  \draw [white, line width=2mm] (#2,#3) to [out=90,in=270] (#1,#4);
  \draw (#2,#3) to [out=90,in=270] (#1,#4);
}

% braiding two strands
% input: x1,x2,y1,y2,label
\def\BraidWithNode(#1,#2,#3,#4,#5){
  \draw (#2,#3) to [out=90,in=270] (#1,#4);
  \draw (#1,#3) to [out=90,in=270] (#2,#4);
  \node (a) at (\avgtwo{#1}{#2},\avgtwo{#3}{#4}) [mynodestyle] {#5};
  %\node (a) at (\avgtwo{#1}{#2},\avgtwo{#3}{#4}) [circle, fill=white, draw, inner sep=1pt] {#5};
}



